No Free Lunch for Defending Against Prefilling Attack by In-Context Learning

The security of Large Language Models (LLMs) has become an important research topic since the emergence of ChatGPT. Though there have been various effective methods to defend against jailbreak attacks, prefilling attacks remain an unsolved and popular threat against open-sourced LLMs. In-Context Learning (ICL) offers a computationally efficient defense against various jailbreak attacks, yet no effective ICL methods have been developed to counter prefilling attacks. In this paper, we: (1) show that ICL can effectively defend against prefilling jailbreak attacks by employing adversative sentence structures within demonstrations; (2) characterize the effectiveness of this defense through the lens of model size, number of demonstrations, over-defense, integration with other jailbreak attacks, and the presence of safety alignment. Given the experimental results and our analysis, we conclude that there is no free lunch for defending against prefilling jailbreak attacks with ICL. On the one hand, current safety alignment methods fail to mitigate prefilling jailbreak attacks, but adversative structures within ICL demonstrations provide robust defense across various model sizes and complex jailbreak attacks. On the other hand, LLMs exhibit similar over-defensiveness when utilizing ICL demonstrations with adversative structures, and this behavior appears to be independent of model size.

==> sections/mainresults_bak.tex <==
%\section{Main Results\label{sec:experimentalresults}}
\section{Experimental Results and Analysis\label{sec:analysis}}

In this section, we introduce experimental results and show detailed analysis of jailbreak defense via ICL with adversative structures by the lens of the existence of safety alignment, \textcolor{red}{GL:todo}
\subsection{The Existence of Safety Alignment}
Figure~\ref{fig:safety_alignment} shows the comparison of ASR between LLMs with and without safety alignment to validate the role of safety alignment which has been the de-facto method for defending against jailbreak attacks. 
Increasing number of prefilling tokens results in more strong prefilling attack~\cite{qi2024safety_shallow}, therefore we report the ASR performance by the lens of the number of prefilling tokens. 
It is obvious that the introduce of safety alignment does not help defend against prefilling jailbreak attacks for both baseline setting an the Adv setting, demonstrating the ineffectiveness of current safety alignment methods. Our finding is in line with that from~\citet{qi2024safety_shallow}.

% \begin{table*}[]
% \small
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccc}

% \hline
% \multicolumn{1}{l}{}                                      & \multicolumn{6}{c}{Rule-based Evaluation}                                                                             \\ \hline
% \multicolumn{1}{l|}{}                                     & falcon-7b     & llama3.1-8b   & llama2-7b     & mistral-7B-v01 & \multicolumn{1}{c|}{vicuna-7b}      & Mean           \\ \hline
% \multicolumn{1}{c|}{Baseline}                             & 92.69         & 73.08         & 29.81         & 92.50          & \multicolumn{1}{c|}{92.12}          & 76.04          \\
% \multicolumn{1}{c|}{Refusal}                                   & 42.31         & 88.85         & 24.23         & 93.08          & \multicolumn{1}{c|}{91.15}          & 67.92          \\
% \multicolumn{1}{c|}{Adv}                          & 4.81          & \textbf{2.88} & 9.23          & 83.65          & \multicolumn{1}{c|}{15.96}          & 23.31          \\
% \multicolumn{1}{c|}{{\color[HTML]{1F1F1F} Adv-mul}} & \textbf{0.77} & 4.42          & \textbf{9.23} & \textbf{60.77} & \multicolumn{1}{c|}{\textbf{15.58}} & \textbf{18.15} \\ \hline
% \multicolumn{1}{l}{}                                      & \multicolumn{6}{c}{Model-based Evaluation}                                                                            \\ \hline
% \multicolumn{1}{l|}{}                                     & falcon-7b     & llama3.1-8b   & llama2-7b     & mistral-7B-v01 & \multicolumn{1}{c|}{vicuna-7b}      & Mean           \\ \hline
% \multicolumn{1}{c|}{Baseline}                             & 86.73         & 22.88         & 27.12         & 95.38          & \multicolumn{1}{c|}{92.50}          & 64.92          \\
% \multicolumn{1}{c|}{Refusal}                                   & 28.27         & 22.31         & 22.69         & 93.27          & \multicolumn{1}{c|}{93.65}          & 52.04          \\
% \multicolumn{1}{c|}{Adv}                          & 1.15          & \textbf{0.58} & \textbf{8.65} & 84.81          & \multicolumn{1}{c|}{15.19}          & 22.08          \\
% \multicolumn{1}{c|}{{\color[HTML]{1F1F1F} Adv-mul}} & \textbf{0.19} & 0.96          & 9.23          & \textbf{63.08} & \multicolumn{1}{c|}{\textbf{15.00}} & \textbf{17.69} \\ \hline
% \end{tabular}%
% }
% \caption{Results on Advbench}
% \label{tab:advbench}
% \end{table*}


% \begin{table*}[]
% \small
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccc}
% \hline
% \multicolumn{1}{l}{}                                      & \multicolumn{6}{c}{Rule-based Evaluation}                                                                                \\ \hline
% \multicolumn{1}{l|}{}                                     & falcon-7b      & llama3.1-8b    & llama2-7b      & mistral-7B-v01 & \multicolumn{1}{c|}{vicuna-7b}      & Mean           \\ \hline
% \multicolumn{1}{c|}{Baseline}                             & 90.00          & 80.00          & 50.00          & 100.00         & \multicolumn{1}{c|}{100.00}         & 84.00          \\
% \multicolumn{1}{c|}{RD}                                   & 57.00          & 76.00          & 41.00          & 97.00          & \multicolumn{1}{c|}{90.00}          & 72.20          \\
% \multicolumn{1}{c|}{AD (Simple)}                          & 36.00          & \textbf{11.00} & 30.00          & 88.00          & \multicolumn{1}{c|}{26.00}          & 38.20          \\
% \multicolumn{1}{c|}{{\color[HTML]{1F1F1F} AD (Multiple)}} & \textbf{10.00} & 17.00          & \textbf{23.00} & \textbf{85.00} & \multicolumn{1}{c|}{\textbf{12.00}} & \textbf{29.40} \\ \hline
% \multicolumn{1}{l}{}                                      & \multicolumn{6}{c}{Model-based Evaluation}                                                                               \\ \hline
% \multicolumn{1}{l|}{}                                     & falcon-7b      & llama3.1-8b    & llama2-7b      & mistral-7B-v01 & \multicolumn{1}{c|}{vicuna-7b}      & Mean           \\ \hline
% \multicolumn{1}{c|}{Baseline}                             & 70.00          & 10.00          & 50.00          & 90.00          & \multicolumn{1}{c|}{90.00}          & 62.00          \\
% \multicolumn{1}{c|}{RD}                                   & 31.00          & 0.00           & 45.00          & 90.00          & \multicolumn{1}{c|}{98.00}          & 52.80          \\
% \multicolumn{1}{c|}{AD (Simple)}                          & \textbf{2.00}  & \textbf{1.00}  & \textbf{25.00} & 84.00          & \multicolumn{1}{c|}{26.00}          & 27.60          \\
% \multicolumn{1}{c|}{{\color[HTML]{1F1F1F} AD (Multiple)}} & \textbf{3.00}  & \textbf{0.00}  & 20.00          & \textbf{82.00} & \multicolumn{1}{c|}{\textbf{10.00}} & \textbf{23.00} \\ \hline
% \end{tabular}%
% }
% \caption{Results on Jailbench}
% \label{tab:jailbench}
% \end{table*}




% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{comment}
\begin{table*}[]

\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\hline
\multicolumn{1}{c|}{\textcolor{red}{AdvBench} |~\textcolor{blue}{Rule}} & falcon-7b     & falcon-11b   & llama2-7b     & llama2-13b      & llama3.1-8b   & llama3.2-3b   & mistral-7B-v01 & vicuna-7b     & vicuna-13b    \\ \hline
\multicolumn{1}{c|}{Baseline}                  & 92.7          & 91.5         & 29.8          & 20.0            & 73.1          & 66.0          & 92.5           & 92.1          & 90.4          \\
\multicolumn{1}{c|}{Refusal}                        & 42.3          & 70.2         & 24.2          & 24.4            & 88.8          & 77.7          & 93.1           & 91.2          & 91.0          \\
\multicolumn{1}{c|}{Adv}                        & 4.8           & \textbf{0.2} & 9.2           & 1.9             & \textbf{2.9}  & 21.5          & 83.7           & 16.0          & 6.9           \\
\multicolumn{1}{c|}{Adv-mul}                    & \textbf{0.8}  & 0.4          & \textbf{9.2}  & \textbf{0.8}    & 4.4           & \textbf{19.6} & \textbf{60.8}  & \textbf{15.6} & \textbf{4.6}  \\ \hline
\textcolor{red}{AdvBench} |~\textcolor{blue}{Model}                     & falcon-7b     & falcon-11b   & llama2-7b     & llama2-13b-chat & llama3.1-8b   & llama3.2-3b   & mistral-7B-v01 & vicuna-7b     & vicuna-13b    \\ \hline
\multicolumn{1}{c|}{Baseline}                  & 86.7          & 94.2         & 27.1          & 17.7            & 22.9          & 30.6          & 95.4           & 92.5          & 91.3          \\
\multicolumn{1}{c|}{Refusal}                        & 28.3          & 63.7         & 22.7          & 21.3            & 22.3          & 21.9          & 93.3           & 93.7          & 86.0          \\
\multicolumn{1}{c|}{Adv}                        & 1.2           & \textbf{0.2} & \textbf{8.7}  & 2.3             & \textbf{0.6}  & \textbf{2.1}  & 84.8           & 15.2          & 6.3           \\
\multicolumn{1}{c|}{Adv-mul}                    & \textbf{0.2}  & 0.4          & 9.2           & \textbf{0.8}    & 1.0           & 2.7           & \textbf{63.1}  & \textbf{15.0} & \textbf{4.0}  \\ \hline
\textcolor{red}{JailBench} |~\textcolor{blue}{Rule}                     & falcon-7b     & falcon-11b   & llama2-7b     & llama2-13b-chat & llama3.1-8b   & llama3.2-3b   & mistral-7B-v01 & vicuna-7b     & vicuna-13b    \\ \hline
\multicolumn{1}{c|}{Baseline}                  & 90.0          & 100.0        & 50.0          & 40.0            & 80.0          & 80.0          & 100.0          & 100.0         & 90.0          \\
\multicolumn{1}{c|}{Refusal}                        & 57.0          & 80.0         & 41.0          & 42.0            & 76.0          & 69.0          & 97.0           & 90.0          & 87.0          \\
\multicolumn{1}{c|}{Adv}                        & 36.0          & 4.0          & 30.0          & \textbf{4.0}    & \textbf{11.0} & 33.0          & 88.0           & 26.0          & 18.0          \\
\multicolumn{1}{c|}{Adv-mul}                    & \textbf{10.0} & \textbf{4.0} & \textbf{23.0} & 5.0             & 17.0          & \textbf{31.0} & \textbf{85.0}  & \textbf{12.0} & \textbf{11.0} \\ \hline
\textcolor{red}{JailBench} | \textcolor{blue}{Model}                    & falcon-7b     & falcon-11b   & llama2-7b     & llama2-13b-chat & llama3.1-8b   & llama3.2-3b   & mistral-7B-v01 & vicuna-7b     & vicuna-13b    \\ \hline
\multicolumn{1}{c|}{Baseline}                  & 70.0          & 100.0        & 50.0          & 30.0            & 10.0          & 60.0          & 90.0           & 90.0          & 80.0          \\
\multicolumn{1}{c|}{Refusal}                        & 31.0          & 80.0         & 45.0          & 37.0            & 0.0           & 72.0          & 90.0           & 98.0          & 78.0          \\
\multicolumn{1}{c|}{Adv}                        & \textbf{2.0}  & 9.0          & 25.0          & 4.0             & 1.0           & 56.0          & 84.0           & 26.0          & 20.0          \\
\multicolumn{1}{c|}{Adv-mul}                    & 3.0           & \textbf{6.0} & \textbf{20.0} & \textbf{3.0}    & \textbf{0.0}  & \textbf{41.0} & \textbf{82.0}  & \textbf{10.0} & \textbf{8.0}  \\ \hline
\end{tabular}%
}
\caption{%Results for Rule-based and Model-based ASR across various models, including the family of LLama, Falcon, Vicuna, and Mistral. We evaluate the models on AdvBench and JailBench, respectively.
\small ASR performance of defense methods across various LLMs. The best performance is highlighted with a bold font. The benchmark is highlighted with a red color, e.g., \textcolor{red}{AdvBench} and \textcolor{red}{Jailbench}. The evaluation metric is highlighted with a blue color, e.g., \textcolor{blue}{Rule} for rule-based ASR, and \textcolor{blue}{Model} for Model-based ASR.
}
\label{tab:my-table}
\end{table*}
\end{comment}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ccccccccc}
\hline
\textbf{GIVEANAME} &\textbf{ Methods} & falcon-7b & falcon-11b & llama2-7b & llama2-13b(-chat) & llama3.1-8b & llama3.2-3b & mistral-7B-v01 & vicuna-7b & vicuna-13b \\ \hline
\multirow{4}{*}{\begin{tabular}{c}
\textcolor{red}{AdvBench}\\[-2pt]\textcolor{blue}{Rule}
\end{tabular}}
& Baseline & 92.7 & 91.5 & 29.8 & 20.0 & 73.1 & 66.0 & 92.5 & 92.1 & 90.4 \\
& Refusal & 42.3 & 70.2 & 24.2 & 24.4 & 88.8 & 77.7 & 93.1 & 91.2 & 91.0 \\
& Adv & 4.8 & \textbf{0.2} & 9.2 & 1.9 & \textbf{2.9} & 21.5 & 83.7 & 16.0 & 6.9 \\
& Adv-mul & \textbf{0.8} & 0.4 & \textbf{9.2} & \textbf{0.8} & 4.4 & \textbf{19.6} & \textbf{60.8} & \textbf{15.6} & \textbf{4.6} \\ \hline
\multirow{4}{*}{\begin{tabular}{c}
\textcolor{red}{AdvBench}\\[-2pt]\textcolor{blue}{Model}
\end{tabular}}
& Baseline & 86.7 & 94.2 & 27.1 & 17.7 & 22.9 & 30.6 & 95.4 & 92.5 & 91.3 \\
& Refusal & 28.3 & 63.7 & 22.7 & 21.3 & 22.3 & 21.9 & 93.3 & 93.7 & 86.0 \\
& Adv & 1.2 & \textbf{0.2} & \textbf{8.7} & 2.3 & \textbf{0.6} & \textbf{2.1} & 84.8 & 15.2 & 6.3 \\
& Adv-mul & \textbf{0.2} & 0.4 & 9.2 & \textbf{0.8} & 1.0 & 2.7 & \textbf{63.1} & \textbf{15.0} & \textbf{4.0} \\ \hline
\multirow{4}{*}{\begin{tabular}{c}
\textcolor{red}{JailBench}\\[-2pt]\textcolor{blue}{Rule}
\end{tabular}}
& Baseline & 90.0 & 100.0 & 50.0 & 40.0 & 80.0 & 80.0 & 100.0 & 100.0 & 90.0 \\
& Refusal & 57.0 & 80.0 & 41.0 & 42.0 & 76.0 & 69.0 & 97.0 & 90.0 & 87.0 \\
& Adv & 36.0 & 4.0 & 30.0 & \textbf{4.0} & \textbf{11.0} & 33.0 & 88.0 & 26.0 & 18.0 \\
& Adv-mul & \textbf{10.0} & \textbf{4.0} & \textbf{23.0} & 5.0 & 17.0 & \textbf{31.0} & \textbf{85.0} & \textbf{12.0} & \textbf{11.0} \\ \hline
\multirow{4}{*}{\begin{tabular}{c}
\textcolor{red}{JailBench}\\[-2pt]\textcolor{blue}{Model}
\end{tabular}}
& Baseline & 70.0 & 100.0 & 50.0 & 30.0 & 10.0 & 60.0 & 90.0 & 90.0 & 80.0 \\
& Refusal & 31.0 & 80.0 & 45.0 & 37.0 & 0.0 & 72.0 & 90.0 & 98.0 & 78.0 \\
& Adv & \textbf{2.0} & 9.0 & 25.0 & 4.0 & 1.0 & 56.0 & 84.0 & 26.0 & 20.0 \\
& Adv-mul & 3.0 & \textbf{6.0} & \textbf{20.0} & \textbf{3.0} & \textbf{0.0} & \textbf{41.0} & \textbf{82.0} & \textbf{10.0} & \textbf{8.0} \\ \hline
\end{tabular}%
}
\caption{\small ASR performance of defense methods across various LLMs.}
\label{tab:my-table}
\end{table*}


\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{figs/sl_rule.png}
        \label{fig:sl-rule}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{figs/sl_model.png}
        \label{fig:sl-model}
    \end{subfigure}
\caption{Results Rule-based~(Left)/Model-based ASR~(Right) on Aligned \& Unaligned Models via AdvBench. We utilized Wizard-Vicuna-13B and Vicuna-13B as the unaligned/aligned models, respectively.}
\label{fig:safety_alignment}
\end{figure*}



\begin{table*}[]
\centering
\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc|cccc}
\hline
\multicolumn{1}{l|}{} & \multicolumn{4}{c|}{Rule-based Evaluation}            & \multicolumn{4}{c}{Model-based Evaluation}            \\ \hline
Falcon-7b             & Prefill     & +AIM       & +EC        & +RS        & Prefill     & +AIM       & +EC        & +RS        \\ \hline
Baseline              & 90          & 70          & 90          & 80          & 70          & 90          & 80          & 50          \\
RD                    & 57          & 76          & 85          & 70          & 31          & 52          & 44          & 37          \\
AD (Multi)            & \textbf{10} & \textbf{47} & \textbf{39} & \textbf{31} & \textbf{3}  & \textbf{30} & \textbf{10} & \textbf{4}  \\ \hline
Llama3.1-8b           & Prefill     & +AIM       & +EC        & +RS        & Prefill     & +AIM       & +EC        & +RS        \\ \hline
Baseline              & 80          & 70          & 90          & 90          & 10          & 70          & 80          & 60          \\
RD                    & 76          & 85          & 86          & 87          & 0           & 79          & 84          & 64          \\
AD (Multi)            & \textbf{17} & \textbf{44} & \textbf{79} & \textbf{76} & \textbf{0}  & \textbf{30} & \textbf{59} & \textbf{53} \\ \hline
Vicuna-8b             & Prefill     & +AIM       & +EC        & +RS        & Prefill     & +AIM       & +EC        & +RS        \\ \hline
Baseline              & 100         & 90          & 90          & 80          & 90          & 100         & 100         & 100         \\
RD                    & 90          & 71          & 88          & 75          & 98          & 93          & 99          & 98          \\
AD (Multi)            & \textbf{12} & \textbf{56} & \textbf{68} & \textbf{56} & \textbf{10} & \textbf{72} & \textbf{75} & \textbf{78} \\ \hline
\end{tabular}%
}
\caption{Results for combining prefilling attacks with other jailbreaking attacks including AIM...}
\label{tab:otherattk}
\end{table*}






==> sections/mechanism.tex <==
\section{Mechanism of Refusal and Adversative Structures\label{sec:mechanism}}

In this section, we first specify the oracle model for defending against prefilling attack by contextual demonstrations, where assuming we can obtain the most relevant demonstrations to the query. By analyzing the Attack Success Rate~(ASR) under the condition of oracle model via JailbreakBench~\cite{chao2024jailbreakbench}, we claim that harmful demonstrations cannot help LLMs to defend against prefilled attacks at all, while adversative demonstrations have huge potential to enable LLMs to be robust to prefilled affirmative tokens related to a harmful query. 

\subsection{Oracle Model}
The goal of ICL-based defense is making LLMs learn to refuse harmful queries via demonstrations $[q_i,a_i]_{i=1}^{c}$. It is important to reveal how each contextual question $q_i$ and contextual answer $a_i$ influence the defending performance. The oracle model for refusal demonstrations can be formulated as $\pi^{ref}_{\theta}\sim\pi_{\theta}(\cdot | x, y_{\leq k}, [x,a*]_{i=1}^{c})$, where the ideal contextual question $q_i$ is the harmful query $x$ itself, and $a*$ is a refusal answer as \textit{I'm sorry I cannot assist with this question}. With respect to the oracle model for adversative demonstration, we denote it as $\pi^{adv}_{\theta}\sim\pi_{\theta}(\cdot | x, y_{\leq k}, [x,y\oplus \hat{a}]_{i=1}^{c})$, where $y$ is true affirmative answer like \textit{Sure. I can help.} And $\hat{a}$ is a transitional sentence like \textit{However, I rethink and I cannot do it.}

\subsection{Refusal \& Adversative Demonstration}
\cref{fig:oracle} presents the results for comparing the ASR for the baseline~(blue bar), the refusal demonstrations~(red bar) and the green demonstrations~(green bar) on Llama-3.1-8B and Mistral-7B-v0.2. Both of these two models are aligned with human values. They are robust to most jailbreaking attacks but remain vulnerable when facing prefilled attack. 

In \cref{fig:oracle}, we observed (1) Compared to the baseline, the oracle model $\pi^{ref}_{\theta}$ for refusal demonstrations do not help to reduce the ASR and even cause the model to be more vulnerable to the prefilling attack. (2) The oracle model $\pi^{adv}_{\theta}$ for adversative demonstrations decreases the ASR with a significant gap compared to the baseline, indicating their huge potential for defending against prefilled attacks. Besides, repeating the ideal demonstration $[x,y\oplus \hat{a}]$ 2/8/16 times~($c=2,8,16$) can also help to decrease the ASR. It gives us an insight that as long as the question $q_{i}$ and the answer $a_{i}$ is semantically similar enough to the query $x$ and prefilling tokens $y$, simply repeating demonstration $[x,y\oplus \hat{a}]$ can help model learn to refuse harmful queries with prefilling jailbreak tokens more deeply. Besides, increasing the prefilled token number $c$ generally increases ASR for the natural and no-demonstration settings, indicating that higher numbers of prefilled tokens can make the models more vulnerable. However, repeating the ideal demonstration $[x, y \oplus a]$ multiple times (as seen with $c = 2, 8, 16$) helps to consistently decrease the ASR, demonstrating a correlation between demonstration repetition and the ability of models to refuse malicious queries more robustly. This pattern suggests that semantic similarity and repeated exposure during the training phase enable the model to learn more nuanced responses than refuse harmful queries effectively.

In the next section, we will study the influence of textual similarity between the demonstrations and input, and analyze how this textual similarity can effect the model's robustness to prefilling attack.

==> sections/practical.tex <==
\section{Performance Landscape\label{sec:practical}}

\begin{table*}[h]
\centering
\begin{tabular}{c|c|c}
\hline
\multicolumn{1}{l|}{}    & Random Sampling & Similarity-based Sampling \\ \hline
No Demonstration         & 0.59            & 0.59                      \\
2 Demonstrations ($c=2$) & 0.68            & 0.62                      \\
Repeat 4 Times ($c=8$)   & 0.53            & 0.53                      \\
Repeat 8 Times ($c=16$)  & \textbf{0.48}   & \textbf{0.43}             \\ \hline
\end{tabular}
\label{tab: mitigate1}
\caption{Migitating the failure case~(Mistral-7B-v02) marked as red in \cref{tab:comparison}, where $k=4$. }
\end{table*}


\begin{table*}
\centering
\begin{tabular}{c|c|c}
\hline
\multicolumn{1}{l|}{}    & Random Sampling                     & Similarity-based Sampling           \\ \hline
No Demonstration         & 0.59                                & 0.59                                \\
2 Demonstrations ($c=2$) & 0.81                                & 0.66                                \\
Repeat 4 Times ($c=8$)   & 0.8                                 & 0.62                                \\
Repeat 8 Times ($c=16$)  & {\color[HTML]{CB0000} \textbf{0.8}} & {\color[HTML]{CB0000} \textbf{0.6}} \\ \hline
\end{tabular}
\label{tab: mitigate2}
\caption{Migitating the failure case~(Mistral-7B-v02) marked as red in \cref{tab:comparison}, where $k=6$. }
\end{table*}


In this section, we provide a performance landscape for leveraging adversative demonstrations for defending against prefilling attacks in partial scenarios . As we introduced in \cref{sec:textualsim}, our pipeline first generates synthetic adversative demonstrations by using unaligned LLM and then randomly samples demonstrations from the data pool $C_{pool}$ can help most models defend against prefilling attack. Besides, similarity-based sampling can be applied to decrease the ASR, if the last layer representations $f_{\theta}(x)$ and $f_{\theta}(q_{i})$ can be accessed. For the failure cases like Mistral-7B-v02, based on our observations in \cref{sec:mechanism} and \cref{sec:textualsim}, we demonstrate that the failures can be alleviated by simply repeating the demonstrations. However, it cannot be fully alleviated since it is not possible to exactly approximate the oracle model.  

\subsection{Comparison Study}
As we have introduced in \cref{sec:mechanism}, we have two sampling methods corresponding to two different practical scenarios: random sampling and similarity-based sampling. We presented the results for the comparison study in \cref{tab:comparison}.

Across all models, the trend consistently shows that the Oracle Model performs best, followed by similarity-based sampling, and finally random sampling. For random sampling, we mark the data as green if it decreases the ASR compared to the baseline, while we mark the data as red if it fails to improve the robustness to the prefilling attack. For Mistral-7B-v02, despite the oracle model being promising, both random sampling and similarity-based sampling fail to defend against the prefilling attack, and even make the situation worse. This case suggests that there is no free lunch for defending against prefilling attack, as despite the oracle model being promising, one still cannot fully control it to be successful.  

The magnitude of this effect and the relative differences vary depending on the model, just as we mentioned in \cref{sec:textualsim} that sensitivity of textual similarity is different among different models. In \cref{tab:comparison}, similarity-based sampling generally performs better than random sampling, but the gap varies by model; it is narrower for Llama models and much wider for Mistral-7B-v0.2, indicating that some models are more sensitive to the textual similarity, which is consistent with our analysis results in \cref{sec:textualsim}.  
% For Mistral-7B-v0.2, the gap between Oracle and Similarity-based Sampling is significant, suggesting the importance of constructing a diverse demonstrations pool that can cover samples similar to the input query. 

\subsection{Mitigating the Failure Case}
\textcolor{red}{\cref{tab: mitigate1} and \cref{tab: mitigate2}} illustrate the results for mitigating the failure case for Mistral-7B-v0.2~(marked as red in \cref{tab:comparison}) by repeating demonstrations to 4 and 8 times. We observe that the effectiveness of repeating strategy is not only related to the averaged textual similarity between query and demonstrations~(Check our claims in \cref{sec:textualsim}), but also related to the prefilling tokens $k$. Although the repeating strategy can decrease the ASR on both $k=4$ and $k=6$, it still cannot mitigate the failure on $k=6$. This phenomenon also indicates that there is no free lunch for prefilling jailbreak defense by ICL.

% The two tables illustrate that Similarity-based Sampling generally outperforms Random Sampling in mitigating failure cases for Mistral-7B-v0.2, especially as the number of repeated demonstrations increases. Across both tables for  k = 4  and  k = 6 , using No Demonstration results in a baseline ASR of 0.59, while adding 2 Demonstrations raises the ASR more significantly for Random Sampling compared to Similarity-based Sampling. Repeating the demonstrations ( c = 8  and  c = 16 ) generally helps reduce ASR, but Similarity-based Sampling shows a larger reduction compared to Random Sampling, particularly with more repetitions (e.g., ASR dropping to 0.43 and 0.60 for  k = 4  and  k = 6 , respectively). The results highlight that careful selection and repetition of demonstrations are crucial for effectively mitigating attack vulnerabilities.


==> sections/sim_analysis.tex <==
\section{Textual Similarity Analysis\label{sec:textualsim}}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/ques_sim_many_shot.png}
        \caption{Few-shot Adversative Demonstrations~($c=2$)}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/ques_sim_few_shot.png}
        \caption{Many-shot Adversative Demonstrations~($c=16$)}
        \label{fig:sub1}
    \end{subfigure}
    \caption{The ASR results for similarity-wise cutting among different LLMs. For each query $x$, we conducted quantile-based discretization with respect to $\sum_{i=1}^{c}s_{x,q_{i}}$. The number of prefilled tokens is set as $k=6$}
    \label{fig:ques_sim}
\end{figure*}

In real-world applications, the oracle model $\pi^{adv}_{\theta}$ is not always doable. For example, most LLM applications may not  allow the developers to access the user input due to privacy concerns. Besides, the oracle model will also cause the overdefense issue on benign queries since directly applying input query to the demonstrations will make the model collapse to refuse everything. 

In this section, we study the topic of defending against prefilling attacks in a more practical scenario in which the LLMs cannot access both the input query $x$ and prefilling tokens $y$. We first introduce our method for how to generate and select the synthetic demonstrations, which serves as a basic pipeline for building ICL-based prefilling attack defense in the particle scenario. By leveraging our generated demonstrations, we observed the effectiveness of ICL-based defense is highly sensitive to the textual similarity between input and demonstration, and rethink the effectiveness of the repeating strategy which can further decrease the ASR under the circumstance of oracle model.

\subsection{Demonstration Generation \& Selection}
% To get a pool for contextual questions as $\{q_{i}\}_{i=1}^{N}$, we select ten different topics according to the JailbreakBench, and use an unaligned model~(e.g., WizardLM-13B-Uncensored) to generate harmful questions related to these topics. Then a ChatGPT-based filter will be applied to remove the duplicated questions and the questions that are judged as not harmful. 
% The detailed flow diagram of the demonstration generation will be shown in the Appendix. 
\textbf{Demonstration Generation.} To obtain a pool of contextual questions denoted as $\{q_{i}\}_{i=1}^{N}$, we start by selecting ten different topics based on the JailbreakBench dataset, which encompasses various sensitive or potentially harmful scenarios intended to test model robustness. Using an unaligned language model—such as WizardLM-13B-Uncensored—we generate harmful questions that are specifically related to these selected topics. Once the questions are generated, a comprehensive filtering step is performed using a ChatGPT-based classifier. This filter serves a dual purpose: first, it identifies and removes any duplicate questions, ensuring a diverse set of prompts within the pool; second, it discards questions that are deemed to lack harmful intent, as determined by the classifier’s judgment criteria. The filtering step is critical to refining the dataset, guaranteeing that only unique and genuinely harmful questions remain, thus enhancing the reliability and quality of subsequent evaluations of model safety and robustness. We denote the demonstration pool as $C_{pool} = \{q_{i},a_{i}\}_{i=1}^{N}$


\textbf{Demonstration Selection.} To investigate the influence of textual similarity, for each query $x$, we select the $c$ most similar questions $\{q_{i}\}_{i=1}^{c}$ based on the similarity metric, and then they are paired with adversative answers. We call this process as \textbf{Similarity-based Selection}. There are many different methods to measure the similarity between input and demonstration~\cite{reimers-2019-sim1,deshpande2023-sim2}. In this work, we use the most direct similarity metric as the cosine similarity between the two last hidden state representations to measure the textual similarity. As what was mentioned in \cref{sec:preliminary}, for the textual similarity between input query $x$ and contextual question $q_{i}$, it can be denoted as $s_{x,q_{i}} = \cos(f_{\theta}(x),f_{\theta}(q_{i}))$, where $f_{\theta}(x)$ and $f_{\theta}(q_i)$ represent the last hidden state embeddings of the input query and contextual question, respectively. This metric captures the degree of semantic overlap between the input and the contextual demonstration, thereby allowing us to identify the most relevant examples to assist with prefilling attack defense.
 
Since each query $x$ may have $c$ different demonstrations selected for it, we calculate the average similarity score to quantify the overall similarity between the input query and the selected demonstrations as $\frac{1}{c}\sum_{i=1}^{c}s_{x,q_{i}}$. By averaging the similarity across all demonstrations, we gain a comprehensive understanding of how representative the selected contextual questions are in relation to the input query. We will explain that $\frac{1}{c}\sum_{i=1}^{c}s_{x,q_{i}}$ serves as a key factor influencing the defence performance.
% Since each query $x$ may have $c$ different demonstrations, we utilize $\frac{1}{c}\sum_{i=1}^{c}s_{x,q_{i}}$ to describe the textual similarity between the demonstrations and the input query.
% In the last step, we applied ChatGPT to generate the affirmative answer for each generated question and added a transitional sentence to make it adversative. The detailed flow diagram of the demonstration generation will be shown in the Appendix.
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/mistralv01_ques.png}
        \caption{Mistral-7B-v0.1}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/llama2_ques.png}
        \caption{Llama2-7B}
        \label{fig:sub1}
    \end{subfigure}
    \caption{ASR vs. Textual Similarity for Mistral-7B-v0.1 and Llama-2-7B models with varying adversarial demonstration number $c$.}
    \label{fig:ques_sim2}
\end{figure*}

\subsection{Sensitivity to Textual Similarity}

We propose a research question as \textit{How does the textual similarity influence the effectiveness of ICL-based prefilling attack defense?} To answer this question, we split the evaluation dataset into four cuts equally by the rank of average textual similarity score $\frac{1}{c}\sum_{i=1}^{c}s_{x,q_{i}}$ in \cref{fig:ques_sim}, and analyze the change of ASR among these four cuts.

As illustrated in \cref{fig:ques_sim}, the average textual similarity $\frac{1}{c}\sum_{i=1}^{c}s_{x,q_{i}}$ increases progressively from cut1 to cut4. We calculate the ASR for each segment and observed that, as the average textual similarity decreases from cut1 to cut4, the ASR also decreases for all four models, with a more significant reduction observed in the many-shot demonstration setting. In addition, compared to the Mistral models~(Mistral-7B-v0.1 and Mistral-7B-v0.1), the Llama models~(Llama-3.1-8B and Llama-2-7B) consistently exhibit the lowest ASR across all cuts in both settings of many-shot and few-shot demonstrations, and their trend of ASR decline from cut1 to cut4 is noticeably smoother. This phenomenon delivers a message that Llama models are less sensitive to the textual similarity compared to mistral models. This implies that Llama models have mode chance to achieve robustness against prefilled attacks compared to Mistral models, especially when the user’s query cannot be used for similarity-based retrieval.

We answer the proposed research question as follows: (1) An increase in textual similarity between the input query and the selected contextual demonstrations leads to a lower Attack Success Rate (ASR), indicating that higher textual similarity may make the model more vulnerable to adversarial attacks. (2) The reduction in ASR is more significant in the many-shot setting compared to the few-shot setting, suggesting that the number of demonstrations plays a significant role in the effectiveness of defense mechanisms.

\begin{table*}[h]
\begin{tabular}{c|c|cccc}
\hline
\multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}     & Llama3.1-8B                 & Llama2-7B                   & Mistral-7B-v01              & Mistral-7B-v02              \\ \hline
                          & No Demonstration          & 0.52                        & 0.5                         & 0.93                        & 0.59                        \\
                          & Oracle Model              & 0.22                        & 0.13                        & 0.12                        & 0.49                        \\
                          & Similarity-based Sampling & 0.37                        & 0.38                        & 0.37                        & 0.62                        \\
\multirow{-4}{*}{$k = 4$} & Random Sampling           & {\color[HTML]{32CB00} 0.42} & {\color[HTML]{32CB00} 0.43} & {\color[HTML]{32CB00} 0.39} & {\color[HTML]{CB0000} 0.68} \\ \hline
                          & No Demonstration          & 0.58                        & 0.42                        & 0.92                        & 0.59                        \\
                          & Oracle Model              & 0.23                        & 0.07                        & 0.12                        & 0.49                        \\
                          & Similarity-based Sampling & 0.36                        & 0.38                        & 0.8                         & 0.66                        \\
\multirow{-4}{*}{$k = 6$} & Random Sampling           & {\color[HTML]{32CB00} 0.38} & {\color[HTML]{32CB00} 0.38} & {\color[HTML]{32CB00} 0.8}  & {\color[HTML]{CB0000} 0.81} \\ \hline
                          & No Demonstration          & 0.74                        & 0.43                        & 0.94                        & 0.63                        \\
                          & Oracle Model              & 0.19                        & 0.07                        & 0.12                        & 0.5                         \\
                          & Similarity-based Sampling & 0.27                        & 0.33                        & 0.91                        & 0.5                         \\
\multirow{-4}{*}{$k = 8$} & Random Sampling           & {\color[HTML]{32CB00} 0.28} & {\color[HTML]{32CB00} 0.34} & {\color[HTML]{32CB00} 0.92} & {\color[HTML]{CB0000} 0.68} \\ \hline
\end{tabular}
\caption{The comparison for ASR among different models~(Llama3.1-8B, Llama2-7B, Mistral-7B-v01, and Mistral-7B-v02) under different numbers of prefilling jailbreak tokens~($k=2,6,8$).}
\label{tab:comparison}
\end{table*}

\subsection{Rethinking the Influence of the Demonstration Number}
Under the circumstance of oracle model (\cref{fig:oracle}), we initially claimed that increasing the number of demonstrations  $c$ would significantly reduce the Attack Success Rate~(ASR). In other words, many-shot demonstration defense definitely has better potential for defending against prefilled attack. However, our experimental results indicate that this claim only holds when the contextual questions are sufficiently similar to the input query. In \cref{fig:ques_sim2}, we illustrate the relationship between textual similarity and ASR for two models—Mistral-7B-v0.1 and Llama-2-7B—under varying numbers of demonstrations $c$. As we increase the demonstration number $c$, selecting the top- c similar contextual questions from the generated data pool $C$ results in a decrease in average textual similarity $\frac{1}{c}\sum_{i=1}^{c}s_{x,q_{i}}$.
 
This observation highlights an important pitfall: the effectiveness of the many-shot adversative demonstration defense compared to the few-shot defense depends on the level of textual similarity. Specifically, many-shot demonstrations only outperform few-shot demonstrations when the textual similarity between the input and contextual questions is sufficiently high. Thus, the strategies of increasing the demonstration number or repeating demonstrations are not universally beneficial. In other words, their success hinges on the availability of highly relevant contextual examples. In the practical scenario, we can somehow alleviate this problem by similarity-based demonstration search in our constructed demonstration pool $C$ if the system is allowed to access the user's query. However, if the user's query is blind to the system due to privacy concerns, we can do nothing to control the quality of the demonstrations but sample the demonstration randomly. We conclude this dilemma as no free lunch in defending against the prefilling attack by in-context learning. Based on this conclusion, we will analyze the performance landscape and check if ICL-based defense can be effective in practical scenarios. 



% In the oracle model~(\cref{fig:oracle}), we claimed that increasing demonstration number $c$ will significantly reduce the ASR. However, we found out this claim only holds for the circumstance when the contextual question is similar enough to the input query. In \cref{fig:ques_sim2}, it shows the relationship between textual similarity and ASR for two different models as Mistral-7B-v0.1 and Llama-2-7B among different demonstrations number $c$. Since we select the top-$c$ similar contextual questions for each query from the generated data pool, its textual similarity $\frac{1}{c}\sum_{i=1}^{c}s_{x,q_{i}}$ drops with the increase of demonstration number $c$. Based on this observation, we claimed that the many-shot adversative demonstration defense only outperforms the few-shot adversative demonstration defense if and only if the textual similarity is high enough.






% Llama-3.1-8B consistently exhibits the lowest ASR across all cuts in both many settings.
% The trend of decline across different cuts is noticeably smoother.



